Restorable Shortest Path Tiebreaking for Edge-Faulty Graphs

The restoration lemma by Afek, Bremler-Barr, Kaplan, Cohen, and Merritt [Dist. Comp. '02] proves that, in an undirected unweighted graph, any replacement shortest path avoiding a failing edge can be expressed as the concatenation of two original shortest paths. However, the lemma is tiebreaking-sensitive: if one selects a particular canonical shortest path for each node pair, it is no longer guaranteed that one can build replacement paths by concatenating two selected shortest paths. They left as an open problem whether a method of shortest path tiebreaking with this desirable property is generally possible. We settle this question affirmatively with the first general construction of restorable tiebreaking schemes. We then show applications to various problems in fault-tolerant network design. These include a faster algorithm for subset replacement paths, more efficient fault-tolerant (exact) distance labeling schemes, fault-tolerant subset distance preservers and $+4$ additive spanners with improved sparsity, and fast distributed algorithms that construct these objects. For example, an almost immediate corollary of our restorable tiebreaking scheme is the first nontrivial distributed construction of sparse fault-tolerant distance preservers resilient to three faults.

==> intro.tex <==
\section{Introduction}

Computation of shortest paths through a network is a basic task in computer science, receiving great theoretical and practical research attention \cite{survey}.
The goal is typically to output a \emph{routing table} $R$, where entry $R_{i, j}$ indicates the next hop along a shortest path starting at node $i$ and ending at node $j$.
An important issue in practical networks is that edges can go down for maintenance, thus changing the shortest paths of the graph and requiring the routing table $R$ to be \emph{restored} in light of these temporary failures.
When this happens, one typically wants to avoid recomputing $R$ from scratch, which can be quite costly.
Rather, the goal is to merely \emph{update} $R$, leveraging the fact that a minor change to the graph will often cause only a minor change in the routing table.

\subsection{Replacement Path Decompositions and Restorable Tiebreaking\label{sec:decomplemma}}

In 2002, Afek, Bremler-Barr, Kaplan, Cohen, and Merritt initiated a systematic study of shortest path restoration.
Their theory had applications for \emph{multiprotocol label switching (MPLS)}, a routing protocol that is notoriously slow to update under topological changes to the underlying graph \cite{ABKCH02}.
Towards an improved methodology for routing updates, they proved the following fundamental theoretical lemma, stating that any \emph{replacement path} avoiding a failed edge is simply the concatenation of two shortest paths in the original graph.

\begin{theorem} [\cite{ABKCM02}] \label{thm:rprestore}
Let $G$ be an undirected unweighted graph, let $e \in E(G)$, and let $\pi(s, t)$ be a shortest path in $G \setminus \{e\}$.
Then there is a node $x \in \pi(s, t)$ such that the $s \leadsto x$ prefix and $x \leadsto t$ suffix of $\pi(s, t)$ are both shortest paths in $G$.
\end{theorem}
%\begin{proof} [Proof]
%Let $x$ be the last node on $\pi(s, t)$ with the property that every $s \leadsto x$ shortest path avoids the deleted edge $e=(u, v)$, and let $y$ be the node immediately following $x$ on $\pi(s, t)$.
%Thus there exists a shortest path $\pi(s, y)$ that includes $e$.
%The prefix $\pi(s, x)$ is automatically a shortest path in $G \setminus \{e\}$; since every shortest $s \leadsto x$ path in $G$ avoids $e$, it must also be a shortest path in $G$.
%So it remains to prove that the same property holds for the suffix $\pi(x, t)$; that is, there is no strictly shorter $x \leadsto t$ path in $G$ that passes through $e$.
%
%\begin{center}
%\begin{tikzpicture}
%\draw [fill=black] (0, 0) circle [radius=0.15];
%\draw [fill=black] (7, 0) circle [radius=0.15];
%%\draw (0, 0) -- (7, 0);
%\node at (0, -0.5) {$s$};
%\node at (7, -0.5) {$t$};
%
%\draw [fill=black] (3, 0) circle [radius=0.15];
%\draw [fill=black] (4, 0) circle [radius=0.15];
%\node at (3.5, 0) {\Huge $\mathbf \times$};
%\node at (3, -0.5) {$u$};
%\node at (4, -0.5) {$v$};
%
%\draw [fill=black] (3, 1) circle [radius=0.15];
%\draw [fill=black] (4, 1) circle [radius=0.15];
%\node at (3, 1.5) {$x$};
%\node at (4, 1.5) {$y$};
%\draw [dashed] plot coordinates {(0, 0) (3, 1) (4, 1) (7, 0)};
%\node [rotate=-21] at (5.8, 0.8) {$\pi(x, t)$};
%\draw (0, 0) -- (3, 1);
%
%\draw plot [smooth] coordinates {(0, 0) (3, 0) (4, 0) (4, 1)};
%\node at (1.5, -0.4) {$\pi(s, y)$};
%\node [rotate=21] at (1.2, 0.8) {$\pi(s, x)$};
%
%\end{tikzpicture}
%\end{center}
%
%To prove this, looking at the $u \leadsto y$ suffix of the shortest path $\pi(s, y)$ and applying the triangle inequality, we have
%$$1 + \dist(v, y) \le \dist(u, x) + 1.$$
%Now looking at the possible $x \leadsto v$ paths, let us compare (1) a path $\pi_1(x, v)$ that walks the edge $(x, y)$ and then travels a shortest $y \leadsto v$ path (hence avoiding $e$) and (2) a path $\pi_2(x, v)$ that travels a shortest $x \leadsto u$ path and then walks the edge $(u, v)$ (hence including $e$).
%The above inequality implies that $|\pi_1(x, v)| \le |\pi_2(x, v)|$.
%Thus, any prefix of a shortest $x \leadsto t$ path in $G$ that includes $e$ may be replaced by an equally-short prefix that avoids $e$, and the lemma follows.
%\end{proof}

While Theorem \ref{thm:rprestore} is the cleanest and seemingly strongest structure theorem proved in \cite{ABKCM02}, the subsequent applications of their restoration theory, such as \cite{?, ?, ?}, have generally not used Theorem \ref{thm:rprestore} directly.
This is due to the premise that one typically wants to apply Theorem \ref{thm:rprestore} in the presence of a precomputed routing table, which implicitly selects a \emph{particular} shortest path for each node pair.
These choices generally spoil Theorem \ref{thm:rprestore}: it is not generally true that there exists any $s \leadsto t$ replacement path formed by concatenating two paths of the form $\pi(s, x), \pi(x, t)$, where these denote the particular $s \leadsto x, x \leadsto t$ shortest paths encoded in the routing.
Thus prior work has abandoned Theorem \ref{thm:rprestore} for weaker structure theorems that enjoy robustness to the shortest path tiebreaking encoded by the routing table.

This paper operates on the front end of Afek et al.'s restoration theory, in the stage where the routing table itself is being designed.
We ask whether Theorem \ref{thm:rprestore}, and its tiebreaking-sensitivity, can be rescued by careful design.
That is:
\begin{center}
\emph{Given an arbitrary undirected unweighted graph, can we compute a routing table $R$ encoding one shortest path for all $n \choose 2$ unordered node pairs in a graph, such that for all nodes $s, t$ and edge $e$, there is a valid $s \leadsto t$ replacement path avoiding $e$ formed by concatenating two selected paths?}
\end{center}

Let us pause briefly to introduce some formalities that help us pose and answer this question.
In network design, it has been recently fruitful to attend to the particular way in which shortest path ties are broken \cite{?, ?}.
This is formalized by \emph{tiebreaking schemes}:
\begin{definition} [Tiebreaking Schemes]
A \emph{tiebreaking scheme} in a graph $G$ is a map $\pi$ such that, for any two nodes $s, t$, $\pi(s, t)$ gives a shortest $s \leadsto t$ path in $G$.
\end{definition}

One can then leverage the combinatorial properties of tiebreaking schemes in algorithms.
For example, a simple property encoded in the above question (since we discuss unordered node pairs) is \emph{symmetry}:
\begin{definition} [Symmetry]
A tiebreaking scheme $\pi$ is \emph{symmetric} if, for all nodes $s, t$, we have $\pi(s, t) = \pi(t, s)$.
\end{definition}

Another property encoded in the above question is that the shortest paths can be encoded in a routing table, meaning that the next hop in the shortest path depends only on the previous node and the destination.
We will discuss a slightly stronger property here:
\begin{definition} [Consistency]
A tiebreaking scheme $\pi$ is \emph{consistent} if, for nodes $s, t, u, v$, if $u, v$ are both in $\pi(s, t)$ in that order, then $\pi(u, v)$ is a contiguous subpath of $\pi(s, t)$.
\end{definition}

Finally, our main new definition is \emph{restorability}, meaning that the tiebreaking implements Theorem \ref{thm:rprestore} as outlined above:
\begin{definition} [Restorability]
A tiebreaking scheme $\pi$ is \emph{restorable} if, for any nodes $s, t$ and edge $e$, there exists a node $x$ such that $\pi(s, x), \pi(t, x)$ together form a valid replacement path, i.e., a shortest $s \leadsto t$ path in the graph $G \setminus \{e\}$.
\end{definition}

So our above question essentially asks whether all undirected unweighted graphs admit a tiebreaking scheme that is simultaneously symmetric, consistent, and restorable.
Our first result is that, unfortunately, the answer is \emph{no}:
\begin{theorem}
A $4$-cycle does not admit a tiebreaking scheme that is simultaneously symmetric and restorable.
\end{theorem}

In fact, up to automorphism a $4$-cycle only has one tiebreaking scheme, and it is easy to verify that it is not restorable.
With this in mind, we next ask what happens if the symmetry axiom is dropped.
This is a bit unusual -- the underlying graph is undirected, but now we allow $\pi(s, t) \ne \pi(t, s)$, even though these paths could be the same in principle.
Our main result is that, surprisingly, this is actually enough to rescue restorability:

\begin{theorem} [Main Result]
Every undirected unweighted graph has a tiebreaking scheme that is simultaneously consistent and restorable.
\end{theorem}

The tiebreaking scheme is fairly simple to implement, and in particular can be computed e.g.\ with a proper implementation of Dijkstra's algorithm.
This unlocks algorithmic applications of Theorem \ref{thm:rprestore}; we use this to prove three new results in the area of fault-tolerant network design, which we overview in the next section.

\subsection{Applications}

Our first applications are to \emph{fault tolerant distance preservers}:
\begin{definition} [Fault Tolerant Subset Distance Preservers]
Given a graph $G = (V, E)$ and a set of ``demand pairs'' $P \subseteq V \times V$, a \emph{distance preserver} of $G, P$ is a subgraph $H$ where $\dist_G(s, t) = \dist_H(s, t)$ for all $(s, t) \in P$.\\

The distance preserver is \emph{$f$-edge fault tolerant ($f$-EFT)} if, for any set of $|F| \le f$ edges, we additionally have that $H \setminus F$ is a distance preserver of $G \setminus F, S$.
\end{definition}

We prove:
\begin{theorem} \label{thm:ssdp}
Given a fixed positive integer $f$, an $n$-node undirected unweighted graph $G = (V, E)$, and a set of source nodes $S \subseteq V$, there is an $f$-EFT distance preserver $H$ of the demand pairs $S \times S$ satisfying
$$|E(H)| = \begin{cases}
O\left( s^{1/2^f} n^{2 - 1/2^f} \right) & f \ne 3\\
O\left( s^{1/3} n^{5/3} \right) & f=3.
\end{cases}$$
\end{theorem}

These preservers can be computed in polynomial time in all parameters.
For comparison, it was proved by Bilo et al.\ \cite{B?} and recently by Bodwin et al.\ \cite{BCPS20} that for any $n$-node undirected weighted graph and source nodes $S$, there is have a $1$-EFT distance preserver on $\Oish(ns)$ edges.
A lower bound of $\Omega(ns)$ was also proved in the latter paper, which holds even if attention is restricted to unweighted graphs.
Hence Theorem \ref{thm:ssdp} is tight in the entire range of parameters in the $1$-fault setting, shaving logs from \cite{B?, BCPS20}.
The more interesting improvements come for larger $f$.
For \emph{weighted} graphs, there are lower bounds implying that no nontrivial construction of $2$-EFT subset distance preservers is possible \cite{?, ?}, and hence these prior methods do not extend beyond one fault (since they are amenable to edge weights).
When $f \ge 2$, no $f$-EFT $S \times S$ distance preservers were known, except those implied by stronger constructions of EFT $S \times V$ distance preservers \cite{Parter, GG, BGPV18}.
Theorem \ref{thm:ssdp} actually works by reduction to these constructions, and it improves its tradeoffs by exactly one fault.
For example, our $3$-EFT $S \times S$ distance preserver has the same asymptotic size as the known $2$-EFT $S \times V$ distance preserver from \cite{Parter?}.


Our next application is a standard use of subset distance preservers in a construction of additive spanners:
\begin{definition} [Fault Tolerant Additive Spanners]
Given a graph $G = (V, E)$, a subgraph $H = (V, E_H \subseteq E)$ is a $+k$ (additive) spanner if we have $\dist_H(s, t) \le \dist_G(s, t) + k$ for all $s, t \in V$.\\

The spanner is $f$-edge fault tolerant (EFT) if, for any set of $|F| \le f$ edges, we additionally have that $H \setminus F$ is a spanner of $G \setminus F$.
\end{definition}

\begin{corollary}
Given a fixed positive integer $f$ and $n$-node undirected unweighted graph $G = (V, E)$, in polynomial time we can compute an $f$-EFT $+4$ spanner $H$ of size
$$|E(H)| = \begin{cases}
O\left( n^{1+1/(1+2^{f-1})} \right) & f \ne 3\\
O\left( n^{7/4} \right) & f = 3.
\end{cases}$$
\end{corollary}

The proof follows a clustering argument that is standard in the area.
For comparison, for $f=1$ our spanner has size $O(n^{3/2})$, which exactly matches the state-of-the-art $1$-EFT $+4$ spanner from \cite{Biloetal}.
The extensions to more faults are new, but see also \cite{?} for constructions where the additive error (rather than the spanner size) scales with the number of faults, and \cite{BGPV18} for related lower bounds.


